Recommending Missed Citations Identified by Reviewers: A New Task, Dataset and Baselines

Citing comprehensively and appropriately has become a challenging task with the explosive growth of scientific publications. Current citation recommendation systems aim to recommend a list of scientific papers for a given text context or a draft paper. However, none of the existing work focuses on already included citations of full papers, which are imperfect and still have much room for improvement. In the scenario of peer reviewing, it is a common phenomenon that submissions are identified as missing vital citations by reviewers. This may lead to a negative impact on the credibility and validity of the research presented. To help improve citations of full papers, we first define a novel task of Recommending Missed Citations Identified by Reviewers (RMC) and construct a corresponding expert-labeled dataset called CitationR. We conduct an extensive evaluation of several state-of-the-art methods on CitationR. Furthermore, we propose a new framework RMCNet with an Attentive Reference Encoder module mining the relevance between papers, already-made citations, and missed citations. Empirical results prove that RMC is challenging, with the proposed architecture outperforming previous methods in all metrics. We release our dataset and benchmark models to motivate future research on this challenging new task.

==> fig_mentions.tex <==
% \begin{figure*}[ht]
%   \centering
%     \subfigure[Recommended citations in the format of reference strings]{\includegraphics[width=0.45\textwidth]{figs/appendix_review1.pdf}}
%     \hspace{0.03\textwidth}
%     \subfigure[Recommended citations in the format of URL links]{\includegraphics[width=0.45\textwidth]{figs/appendix_review2.pdf}} \\
%     \subfigure[Recommended citations in the format of short phrases]{\includegraphics[width=0.45\textwidth]{figs/appendix_review3.pdf}}
%     \hspace{0.03\textwidth}
%     \subfigure[Recommended citations in the format of model names with metadata]{\includegraphics[width=0.45\textwidth]{figs/appendix_review4.pdf}} \\
%     \subfigure[Mentions of already cited papers via metadata]{\includegraphics[width=0.45\textwidth]{figs/appendix_review5.pdf}}
%     \hspace{0.03\textwidth}
%     \subfigure[Mentions of already cited papers via index]{\includegraphics[width=0.45\textwidth]{figs/appendix_review6.pdf}}
%   \caption{Examples of mentions of papers appeared in reviews. Italic and colored texts represent papers mentioned in reviews, among which, enclosed by the dashed border, are those reviewers recommend citing. Underlined and bolded texts indicate reasons why those citations are missed and necessary.}
%     \label{fig:app:reviews}
%     \vspace{0.2in}
% \end{figure*}
